Subgraph centrality and walk-regularity

Matrix-based centrality measures have enjoyed significant popularity in network analysis, in no small part due to our ability to rigorously analyze their behavior as parameters vary. Recent work has considered the relationship between subgraph centrality, which is defined using the matrix exponential $f(x) = \exp(x)$, and the walk structure of a network. In a walk-regular graph, the number of closed walks of each length must be the same for all nodes, implying uniform $f$-subgraph centralities for any $f$ (or maximum $f$-$\textit{walk entropy}$). We consider when non--walk-regular graphs can achieve maximum entropy, calling such graphs $\textit{entropic}$. For parameterized measures, we are also interested in which values of the parameter witness this uniformity. To date, only one entropic graph has been identified, with only two witnessing parameter values, raising the question of how many such graphs and parameters exist. We resolve these questions by constructing infinite families of entropic graphs, as well as a family of witnessing parameters with a limit point at zero.

==> repeated-lemmas/lemma-adj-bound.tex <==
Let $\mA$ be the adjacency matrix for an unweighted, loopless, undirected graph.
Then for each $\ell \in \mathbb{N}^+$ we have $\mA^{\ell}_{jj} \leq (n-1)^{\ell-1}$ for all $j$.


==> repeated-lemmas/lemma-split-power.tex <==
Let $G$ be a deceptive graph with adjacency matrix $\mA$, and let $\vvd{\ell}_j = (\mA^\ell)_{jj}$.
Then there must exist at least two distinct walk-classes for $G$, labelled $w_1$ and $w_2$, and some $s\in \mathbb{N}$ such that for any pair of nodes, 1 and 2, from the two walk classes, $1 \in w_1$ and $2 \in w_2$, we have
    \begin{enumerate}[nolistsep]
        \item[(1)]$\vvd{s}_1 < \vvd{s}_2$;
        \item[(2)]$\vvd{\ell}_1 \geq \vvd{\ell}_2$ for all integers $2 \leq \ell < s$; and
        \item[(3)]$\vvd{h}_1 > \vvd{h}_2$ for at least one power $h < s$.
    \end{enumerate}


==> sec-flip-flop.tex <==
We want to understand when nodes with distinct walk structures can be assigned the same score by a centrality measure --- we call this occurrence a \emph{centrality collision}, or simply a collision.
More precisely, let $G$ be a connected, non--walk-regular graph, and let $\{w_j\}$ be any collection of distinct walk-classes in $G$.
We want to know when we can construct a PPSC function $f(x)$ such that $f(\mA)_{ii}$ is the same for all nodes in the classes $\{w_j\}$;
we say that the walk-classes $\{w_j\}$ \emph{collide} under $f$, and that $f$ \emph{induces a collision} at $\{w_j\}$.
Observe that a graph is $f$-entropic precisely when there exists a function $f$ that induces a collision at all of its walk-classes.

In the remainder of the section, we give a sufficient condition for a graph for the existence of a collision-inducing PPSC function on that graph (Corollary~\ref{cor:pos-suff-condition});
the sufficient condition generalizes to apply to entropic graphs.
Additionally, this leads to a related sufficient condition for concluding that a graph is not $f$-entropic for any function $f$ (Corollary~\ref{cor:walk-class-lin-sys}).
Finally, as an application of our theory, in Section~\ref{sec:spider-torus} we present a graph with three walk-classes which we prove is $f$-entropic using Corollary~\ref{cor:pos-suff-condition}.
This is interesting because previously all known $f$-entropic graphs had only two walk-classes.

\subsection{Sufficient condition for centrality collisions}\label{sec:suff-condition}
Given a collection $\{w_j\}$ of distinct walk-classes in a graph $G$, we would like an easily computable condition that characterizes whether there exists some PPSC function $f$ that induces a collision at $\{w_j\}$.
Here we present a practically computable sufficient condition for such a function's existence.
Interestingly, the condition connects a question about nodes' walk-classes to Farkas's Lemma on nonnegative solutions to linear equations.

\begin{theorem}\label{thm:pos-suff-condition}
    Let graph $G$ have walk matrix $\mW$ and adjacency matrix $\mA$.
    Given $\vb > 0$, if there exists $\vx > 0$ such that $\mW\vx = \vb$, then there exists a PPSC function $f(x)$ such that $\diag(f(\mA)) = \vb$.
\end{theorem}
\begin{proof}
    Assume $\vx > 0$ and $\mW\vx =  \vb$.
    Let $m$ be the degree of the minimal polynomial of $\mA$.
    For each index $k \geq m$ we can use the minimal polynomial of $\mA$ to produce a set of coefficients $\{ p_{k,j} \}_{j=0}^{m-1}$ such that
    $\mA^k = \sum_{j=0}^{m-1} p_{k,j} \mA^j$.
    This will enable us to collapse all terms $\mA^k$ for $k\geq m$ into just the first $m-1$ terms $\{\mA^j\}_{j=0}^{m-1}$.
    Before collapsing, we adjust the coefficients $p_{k,j}$ so that they can be put into certain convergent sums.

    For each $j$, construct a sequence $\{s_{j,k}\}_{k=m}^{\infty}$ so that $\left(\sum_{k=m}^{\infty} p_{k,j} s_{j,k} \right)$ converges to some positive value $c_j$. One such sequence is $s_{j,k} = 2^{-k} |p_{k,j}^{-1}|$; if $p_{k,j} = 0$ then instead use $2^{-k}$.
    Note that each $s_{j,k}$ is positive. Next, for each $k$ define $c_k = \min\{  s_{j,k} | j=0,\cdots,m-1 \}$. Then we have that $\left( \sum_{k=m}^{\infty} p_{k,j} c_k \right)$ converges, for each $j$.
    Using $s_{j,k} = 2^{-k} |p_{k,j}^{-1}|$, we have $|p_{k,j}c_k| \leq 2^{-k}$, and so the magnitude of the sum $\sum_{k=m}^{\infty} p_{k,j} c_k$ is bounded above by $\sum_{k=m}^{\infty} 2^{-k}$.

    Finally, for $j=0, \cdots, m-1$, choose $c_j = x_j - \left( \sum_{k=m}^{\infty} p_{k,j} c_k \right)$.
    If any of these $c_j$ is negative, then choose $\{ c_k \}_{k=m}^{\infty}$ smaller so that the values $c_j = x_j - \left( \sum_{k=m}^{\infty} p_{k,j} c_k \right)$ are positive. This is possible because the $c_k$ can be chosen as close to 0 as we like, and $x_j > 0$ by assumption.
    The end result is that any positive solution $\vx$ to $\mW\vx = \vb$ enables us to equate
    \[
        \sum_{j=0}^{m-1} x_j \diag(\mA^j) \hspace{3pt} =
        \hspace{3pt} \diag\left( \sum_{j=0}^{m-1} x_j \mA^j \right)
            = \hspace{3pt} \diag\left( \sum_{j=0}^{m-1} \left( c_j +  \sum_{k=m}^{\infty} p_{k,j} c_k \right) \mA^j \right).
    \]
    Rearranging, we have $\vb = \diag\left( \sum_{j=0}^{m-1} c_j \mA^j +  \sum_{j=0}^{m-1}\sum_{k=m}^{\infty} p_{k,j} c_k \mA^j \right)$.
    We observe
    \[
       \sum_{j=0}^{m-1} \left( \sum_{k=m}^{\infty} p_{k,j} c_k \right) \mA^j
     \hspace{3pt} = \hspace{3pt}
       \sum_{k=m}^{\infty} c_k \sum_{j=0}^{m-1} p_{k,j}  \mA^j
     \hspace{3pt} = \hspace{3pt}
        \sum_{k=m}^{\infty} c_k \mA^k .
    \]
    Thus, $\vb$ equals $\diag(f(\mA))$ for a PPSC function $f(x)$.
\end{proof}

Note that if we restrict to a subset $S$ of rows of the equation $\mW\vx = \ve$ corresponding to a subset of walk-classes,
then by Theorem~\ref{thm:pos-suff-condition} a positive solution $\vx$ to $\mW_S\vx = \ve$ gives a PPSC function $f$ that induces a collision at the walk-classes contained in $S$.

\begin{corollary}\label{cor:pos-suff-condition}
  Given a graph $G$ with walk matrix $\mW$ and adjacency matrix $\mA$, fix any subset $W = \{w_j\}$ of walk-classes for $G$ and let $J$ be the set of all row indices of $\mW$ corresponding to nodes in the walk-classes in $W$.
  If the linear system $\mW_J\vx = \ve$ has a solution $\vx > 0$, then there exists a PPSC function $f$ that induces a collision at all the walk-classes in $W$.
  That is, there is a constant $c$ such that $f(\mA)_{ii} = c$ for all $i \in w_j \in W$.
\end{corollary}

The above results show that a solution to a particular linear program guarantees that a collision-inducing function exists.
On the other hand, the converse---whether the existence of a collision-inducing PPSC function guarantees the existence of a positive solution to $\mW\vx=\ve$ --- remains an open question.
Lastly, we remark that the above proof shows that if an entropic function exists for $G$ then $\mW\vx = \ve$ is consistent.

\begin{corollary}\label{cor:walk-class-lin-sys}
  Given a graph $G$ with walk matrix $\mW$,
  if the linear system $\mW\vx = \ve$ is inconsistent then $G$ is non--walk-regular and not entropic.
\end{corollary}

\paragraph{Connection to Farkas's Lemma}
We remark that for the linear system in Corollary~\ref{cor:pos-suff-condition} to have a positive solution, it is necessary that the system $\mW\vx=\ve$ satisfies the well-known Farkas's Lemma~\cite{Farkas1902}.
Farkas's Lemma says that a general linear system $\mM\vx = \vb$ has a solution $\vx\geq 0$ if and only if no $\vy$ exists such that $\vy^T\vb < 0$ and $\vy^T\mM \geq0$.
In our restricted setting, where $\mW$ is nonnegative and the right-hand side is $\ve$, we derive a more specific, necessary condition for Farkas's Lemma to hold---and, therefore, a necessary condition for a positive solution to exist in Corollary~\ref{cor:pos-suff-condition}.
However, this novel condition does not have an intuitive interpretation in the context of centrality and walk-classes, and so we defer further discussion to the appendix.


\subsection{A concrete application}\label{sec:spider-torus}

Figure~\ref{fig:spidertorus} displays an $f$-entropic graph, $ST(4,2,[5,3])$, which we call a ``spider torus'', that has exactly three walk-classes.
The center nodes from the spider graphs form the first walk-class, the outer/inner nodes of the spider graphs (labelled with subscripts 1/2) form the second/third. We experimentally verified the graph depicted, $ST(4,2,[5,3])$, to be $f$-entropic using Corollary~\ref{cor:pos-suff-condition}, as implemented in our software package~\cite{spiderdonuts_v1.0.0}.

\begin{figure}[!ht]
  \centering
  \resizebox{0.9\linewidth}{!}{\input{./figures/spidertorus.tex}}
  \caption{
      \emph{(Left)} A spider graph of degree 4 and length 2, denoted $S(4,2)$.
      \emph{(Center)} A ``(4, 2, [3]) spider cycle'', denoted $SC(4,2,[3])$, consists of three copies of $S(4,2)$ such that the three copies of each outer-most node (with label $t_1$ for $t \in \{u,v,w,x\}$)  are connected in a cycle.
      \emph{(Right)} A ``(4, 2, [5, 3]) spider torus'', denoted $ST(4,2,[5,3])$, consists of five copies of $SC(4,2,[3])$ with cycles connecting each set of five inner nodes of the spider legs (with label $t_2$ for $t \in \{u,v,w,x\}$).  $ST(4,2,[5,3])$ has three walk-classes and can be shown to be $f$-entropic using Corollary~\ref{cor:pos-suff-condition}.
  }\label{fig:spidertorus}
\end{figure}

